Emergent Response Planning in LLMs

In this work, we argue that large language models (LLMs), though trained to predict only the next token, exhibit emergent planning behaviors: $\textbf{their hidden representations encode future outputs beyond the next token}$. Through simple probing, we demonstrate that LLM prompt representations encode global attributes of their entire responses, including $\textit{structure attributes}$ (e.g., response length, reasoning steps), $\textit{content attributes}$ (e.g., character choices in storywriting, multiple-choice answers at the end of response), and $\textit{behavior attributes}$ (e.g., answer confidence, factual consistency). In addition to identifying response planning, we explore how it scales with model size across tasks and how it evolves during generation. The findings that LLMs plan ahead for the future in their hidden representations suggest potential applications for improving transparency and generation control.

==> components/4_experiment_results_old.tex <==
% stucture: in-dataset
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_ultrachat_spearman_part.pdf}
        \caption{In-dataset response length prediction results on Ultrachat.}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_gsm8k_spearman_part.pdf}
        \caption{In-dataset reasoning steps prediction on GSM8k.}
    \end{subfigure}
    \caption{In-dataset results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_inDataset}
\end{figure*}


% stucture: cross-dataset
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_ultrachat_To_alpaca_eval_spearman_part.png}
        \caption{Cross-dataset generalization results for response length (Ultrachat$\rightarrow$AlpacaEval).}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_gsm8k_To_MATH_spearman_part.png}
        \caption{Cross-dataset generalization results for reasoning steps (GSM8k$\rightarrow$MATH).}
    \end{subfigure}
    \caption{Cross-dataset generalization results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_crossDataset}
\end{figure*}

% stucture: layer-wise heatmap
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_layerHeatmap_ultrachat_spearman.pdf}
        \caption{Layer-wise results for response length.}
        % \label{fig:exp_}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \\
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_layerHeatmap_gsm8k_spearman.pdf}
        \caption{Layer-wise results for reasoning steps.}
    \end{subfigure}
    \caption{Layer-wise results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_layerWise}
\end{figure*}



% structure: hidden_size
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_ultrachat_spearman.pdf}
        \caption{Ultrachat}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_gsm8k_spearman.pdf}
        \caption{gsm8k}
    \end{subfigure}
    \caption{Hidden size analysis on ultrachat and gsm8k, spearman correlation as metric}
    \label{fig:exp_statistical_hiddensize}
\end{figure*}




%%%%%%%%%%%%%% content
% content: in-dataset
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_TinyStories_f1_score.pdf}
        \caption{In-dataset character choices prediction results on TinyStories.}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_commonsense_qa_f1_score.pdf}
        \caption{In-dataset multiple-choice answers on CommonsenseQA.}
    \end{subfigure}
    \caption{In-dataset results for character choices prediction and multiple-choice answers prediction.}
    \label{fig:exp_content_inDataset}
\end{figure*}

% content: cross-dataset
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_TinyStories_To_ROCStories_f1_score.pdf}
        \caption{Cross-dataset generalization results for character choices (TinyStories$\rightarrow$ROCStories).}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_commonsense_qa_To_social_iqa_f1_score.pdf}
        \caption{Cross-dataset generalization results for multiple-choice answers (CommonsenseQA$\rightarrow$SocialIQA).}
    \end{subfigure}
    \caption{Cross-dataset generalization results for character choices prediction and multiple-choice answers prediction.}
    \label{fig:exp_content_crossDataset}
\end{figure*}

% content: layer-wise heatmap
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_layerHeatmap_TinyStories_f1_score.pdf}
        \caption{Layer-wise results for character choices.}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \\
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_layerHeatmap_commonsense_qa_f1_score.pdf}
        \caption{Layer-wise results for multiple-choice answers.}
    \end{subfigure}
    \caption{Layer-wise results for character choices prediction and multiple-choice answers prediction.}
    \label{fig:exp_content_layerWise}
\end{figure*}

% content: hidden_size
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_TinyStories_f1_score.pdf}
        \caption{TinyStories}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_commonsense_qa_f1_score.pdf}
        \caption{CommonsenseQA}
    \end{subfigure}
    \caption{Hidden size analysis on TinyStories and CommonsenseQA, F1 score as metric}
    \label{fig:exp_statistical_hiddensize}
\end{figure*}


%%%%%%%%%% behavior




\section{Experimental Results}
% \section{Feature Existence: Systematic Evidence from Multi-model, Multi-task Analysis}

In this section, we present experimental results across six tasks, showing that LLM hidden prompt representations encode rich information about upcoming responses and can be used to probe and predict global response attributes.



\subsection{Structure Attributes: Response Length Prediction and Reasoning Steps Prediction}


\textbf{Insight 1: Probes reveal strong linear correlations between predicted and target values, with fine-tuned models showing superior performance.} 
Fig.~\ref{fig:exp_structure_inDataset} shows in-dataset predictions for response length and reasoning steps on test splits. Fine-tuned models exhibit strong linear correlations with ground truth on the test split, clustering around $y=x$, while base models show weaker but still positive correlations. This indicates that \textbf{(1)} model representations encode response length and reasoning step information, and \textbf{(2)} fine-tuning strengthens these patterns, consistent with base models' weaker grasp of response boundaries.


\textbf{Insight 2: The learned patterns well-generalize across datasets.} Fig.~\ref{fig:exp_structure_crossDataset} shows cross-dataset results using probes trained and evaluated on different datasets. While prediction accuracy decreases compared to in-dataset testing, predictions maintain strong correlation with target labels, or even clustering near $y=x$, though this correlation is notably weaker for base models compared to their fine-tuned counterparts. \textbf{This suggests the probes capture both dataset-specific and generalizable task-related patterns.}

\textbf{Insight 3: Structure attribute patterns peak in middle layers for all models.}
Fig.~\ref{fig:exp_layerHeatmap_ultrachat} shows layer-wise pattern saliency through average probe performance (Spearman coefficient), using optimal hidden size across seeds. The results reveal a consistent pattern across both tasks: \textbf{weak performance in early layers, peaks in middle layers, and decline in final layers}. This suggests that \textbf{(1)} response length information accumulates through early layers, peaks in middle layers, then partially diminishes, and \textbf{(2)} attributes emerge through complex layer-wise transformations rather than simple vocabulary statistics.

\textbf{Insight 4: Structure attribute patterns can be extracted adequately by simple and shallow MLPs.} Fig.~\ref{fig:exp_statistical_hiddensize} plots the average probe performance (Spearman coefficient) across layers against hidden size, showing performance plateaus around hidden size 64. This suggests these patterns are readily extractable with simple probing architectures.















\subsection{Content Attributes: Character Choices and Multiple-Choice Answers}

\textbf{Insight 5: Content attribute patterns demonstrate robust classification performance, cross-dataset generalization, and accessibility.} Probing experiments on content attributes parallel our structure attribute findings: \textbf{(1)} Both base and fine-tuned models encode content information significantly above random baselines in in-dataset evaluation, \textbf{(2)} probes maintain above-baseline performance in cross-dataset settings, and \textbf{(3)} content patterns, like structure attributes, can be effectively extracted using simple MLPs with hidden size 32.

\textbf{Insight 6: Content attribute patterns peak in late layers.} Fig.~\ref{fig:exp_layerHeatmap_TinyStories} shows layer-wise pattern saliency using F1 scores, revealing that content attribute performance either remains low until late layers or gradually increases to peak in final layers, contrasting with the mid-layer peaks observed for structure attributes.


 
% \begin{figure*}[tb!] 
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_basicResults_TinyStories_f1_score.pdf}
%         \caption{TinyStories}
%         \label{fig:exp_basicResults_TinyStories}
%     \end{subfigure}
%     \hfill  % Creates horizontal spacing between subfigures
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_basicResults_commonsense_qa_f1_score.pdf}
%         \caption{commonsense\_qa}
%         \label{fig:exp_basicResults_commensense_qa}
%     \end{subfigure}
%     \caption{Results on TinyStories and commonsense\_qa, l1 score as metric}
%     \label{fig:exp_statistical_ContentResults}
% \end{figure*}

% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/exp_generalizationResults_TinyStories_To_ROCStories_f1_score.pdf}
%     \caption{Generalization test from TinyStories to ROCStories on character choices task.}
%     \label{fig:exp_generalization_TinyStories}
% \end{figure}

% \begin{figure*}[tb!]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/exp_layerHeatmap_TinyStories_f1_score.pdf}
%     \caption{Layer-wise F1 score distribution across different language models on the TinyStories dataset. The heatmap shows F1 scores for each layer (x-axis) of various model architectures. Higher scores (darker red) indicate better performance. The results demonstrate that performance generally improves in higher layers, with most models showing peak F1 scores in their later layers.}
%     \label{fig:exp_layerHeatmap_TinyStories}
% \end{figure*}


% \begin{figure*}[tb!] 
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_TinyStories_f1_score.pdf}
%         \caption{TinyStories}
%         % \label{fig:exp_basicResults_ultrachat}
%     \end{subfigure}
%     \hfill  % Creates horizontal spacing between subfigures
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_commonsense_qa_f1_score.pdf}
%         \caption{commonsense\_qa}
%         % \label{fig:exp_basicResults_gsm8k}
%     \end{subfigure}
%     \caption{Hidden size analysis on TinyStories and commonsense\_qa, f1 score as metric}
%     \label{fig:exp_content_hiddensize}
% \end{figure*}





\subsection{Behavior Attributes: Answer Confidence and Factual Consistency}

\textbf{Insight 7: Behavior attribute patterns exhibit strong classification accuracy, cross-dataset transferability, and accessibility.} Probing experiments on behavior attributes parallel our previous findings: \textbf{(1)} Both base and fine-tuned models encode behavior information (Fig.~\ref{fig:exp_main_behavior_inDataset}), \textbf{(2)} probes maintain above-baseline performance when transferring from MedMCQA to ARC-Challenge (Fig.~\ref{fig:exp_main_behavior_crossDataset}), and \textbf{(3)} behavior patterns, like structure and content attributes, can be effectively extracted using simple MLPs with hidden size around 32 (Fig.~\ref{fig:exp_main_behavior_hiddenSize}).


\textbf{Insight 8: Behavior attribute patterns accumulate and peak in different layers across models.} Fig.~\ref{fig:exp_main_behavior_layerWise} reveals that behavior patterns form and peak at model-specific layers, suggesting diverse representational strategies for behavior attributes.


% \begin{figure*}[tb!] 
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_basicResults_medmcqa_f1_score.pdf}
%         \caption{medmcqa}
%         % \label{fig:exp_basicResults_medmcqa}
%     \end{subfigure}
%     \hfill  % Creates horizontal spacing between subfigures
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_basicResults_CREAK_f1_score.pdf}
%         \caption{CREAK}
%         % \label{fig:exp_basicResults_CREAK}
%     \end{subfigure}
%     \caption{Results on medmcqa and CREAK, l1 score as metric}
%     \label{fig:exp_main_behavior_inDataset}
% \end{figure*}

%  \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/exp_generalizationResults_medmcqa_To_ai2_arc-Challenge_f1_score.pdf}
%     \caption{Generalization test from medmcqa to Challenge set of ai2\_arc on answer confidence task.}
%     \label{fig:exp_main_behavior_crossDataset}
% \end{figure}

% \begin{figure*}[tb!]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/exp_layerHeatmap_medmcqa_f1_score.pdf}
%     \caption{Layer-wise F1 score distribution across different language models on the medmcqa dataset. The heatmap shows F1 scores for each layer (x-axis) of various model architectures. Higher scores (darker red) indicate better performance. The results demonstrate that performance generally improves in higher layers, with most models showing peak F1 scores in their later layers.}
%     \label{fig:exp_main_behavior_layerWise}
% \end{figure*}

% \begin{figure*}[tb!] 
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_medmcqa_f1_score.pdf}
%         \caption{medmcqa}
%         % \label{fig:exp_basicResults_ultrachat}
%     \end{subfigure}
%     \hfill  % Creates horizontal spacing between subfigures
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_CREAK_f1_score.pdf}
%         \caption{CREAK}
%         % \label{fig:exp_basicResults_gsm8k}
%     \end{subfigure}
%     \caption{Hidden size analysis on medmcqa and CREAK, f1 score as metric}
%     \label{fig:exp_main_behavior_hiddenSize}
% \end{figure*}



% \subsection{Insights Across Tasks and Attribute Types}
% \textbf{Insight 9: Emergent planning exhibits.} xxx


% \textbf{Insight 10: Different attributes types are mainly decoded in different model layers.} Structure attributes are mainly decoded in the middle layers; content and behavior attributes peaks at finally layers.



==> components/experiments_old.tex <==
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_ultrachat_spearman.png}
        \caption{In-dataset response length prediction results on Ultrachat.}
        % \label{fig:exp_basicResults_ultrachat}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \\
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_gsm8k_spearman.png}
        \caption{In-dataset reasoning steps prediction on GSM8k.}
        % \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{In-dataset results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_inDataset}
\end{figure*}

\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_ultrachat_To_alpaca_eval_spearman.png}
        \caption{Cross-dataset generalization results for response length (Ultrachat$\rightarrow$AlpacaEval).}
        % \label{fig:exp_}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \\
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_gsm8k_To_MATH_spearman.png}
        \caption{Cross-dataset generalization results for reasoning steps (GSM8k$\rightarrow$MATH).}
        % \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{Cross-dataset generalization results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_crossDataset}
\end{figure*}

\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_ultrachat_To_alpaca_eval_spearman.png}
        \caption{Cross-dataset generalization results for response length (Ultrachat$\rightarrow$AlpacaEval).}
        % \label{fig:exp_}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \\
    \begin{subfigure}[b]{0.95\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_generalizationResults_gsm8k_To_MATH_spearman.png}
        \caption{Cross-dataset generalization results for reasoning steps (GSM8k$\rightarrow$MATH).}
        % \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{Cross-dataset generalization results for response length prediction and reasoning steps prediction.}
    \label{fig:exp_structure_crossDataset}
\end{figure*}

\section{Experimental Results}
% \section{Feature Existence: Systematic Evidence from Multi-model, Multi-task Analysis}

In this section, we present experimental results across six tasks, showing that LLM hidden prompt representations encode rich information about upcoming responses and can be used to probe and predict global response attributes.
% In this section, we design tasks to prove the feasibility of probing and predicting future response attributes using hidden features. 
% The tasks fall into three categories: \textbf{1)} structure attributes, which capture response-level metrics like total token length; \textbf{2)} content attributes, which track specific words that may appear anywhere in the response; and \textbf{3)} behavior attributes, which require external ground truth labels, such as answer accuracy.


\subsection{Structure Attributes: Response Length Prediction and Reasoning Steps Prediction}

%\textbf{Task Settings.} We describe our data collection and labeling methods for two regression tasks, where we predict structure-related quantities at different positions within the response. For response length prediction, we use 5k questions from the UltraChat dataset and calculate the remaining token count needed to complete each response at various prediction points using the model's tokenizer. For reasoning steps prediction, we use 5k questions from GSM8K and prompt language models to solve problems in a step-by-step manner, measuring the number of remaining steps needed to reach the final answer at different stages of the solution process.

% \textbf{Task settings.} Both response length and reasoning steps are regression tasks where predictions should be positively related to target values, closely match them, and ideally demonstrate a linear y=x relationship. For response length, we use 5K UltraChat questions (in-dataset) and 1k instructions from AlpacaEval dataset (cross-dataset). For reasoning steps, we evaluate on 5K GSM8K questions. We conduct in-dataset evaluation for both tasks, with further analysis focusing on the response length task. All results are averaged across three random seeds.

\textbf{Insight 1: Probes reveal strong linear correlations between predicted and target values, with fine-tuned models showing superior performance.} 
Fig.~\ref{fig:exp_structure_inDataset} shows in-dataset predictions for response length and reasoning steps on test splits. Fine-tuned models exhibit strong linear correlations with ground truth on the test split, clustering around $y=x$, while base models show weaker but still positive correlations. This indicates that \textbf{(1)} model representations encode response length and reasoning step information, and \textbf{(2)} fine-tuning strengthens these patterns, consistent with base models' weaker grasp of response boundaries.


\textbf{Insight 2: The learned patterns well-generalize across datasets.} Fig.~\ref{fig:exp_structure_crossDataset} shows cross-dataset results using probes trained and evaluated on different datasets. While prediction accuracy decreases compared to in-dataset testing, predictions maintain strong correlation with target labels, or even clustering near $y=x$, though this correlation is notably weaker for base models compared to their fine-tuned counterparts. \textbf{This suggests the probes capture both dataset-specific and generalizable task-related patterns.}

\textbf{Insight 3: Structure attribute patterns peak in middle layers for all models.}
Fig.~\ref{fig:exp_layerHeatmap_ultrachat} shows layer-wise pattern saliency through average probe performance (Spearman coefficient), using optimal hidden size across seeds. The results reveal a consistent pattern across both tasks: \textbf{weak performance in early layers, peaks in middle layers, and decline in final layers}. This suggests that \textbf{(1)} response length information accumulates through early layers, peaks in middle layers, then partially diminishes, and \textbf{(2)} attributes emerge through complex layer-wise transformations rather than simple vocabulary statistics.

\textbf{Insight 4: Structure attribute patterns can be extracted adequately by simple and shallow MLPs.} Fig.~\ref{fig:exp_statistical_hiddensize} plots the average probe performance (Spearman coefficient) across layers against hidden size, showing performance plateaus around hidden size 64. This suggests these patterns are readily extractable with simple probing architectures.

% \textbf{In-dataset results.} We evaluate model performance on both tasks using different train-test splits on UltraChat and GSM8K datasets. As shown in Fig.~\ref{fig:exp_statistical_BasicResults},  fine-tuned models demonstrate a strong linear correlation between predicted and real labels, clustering tightly around $y=x$. In contrast, base models generally show higher variance and weaker correlation, indicating systematic prediction biases.


% \textbf{Cross-dataset generalization results.} We evaluate cross-dataset generalization for response length by applying probes trained on the UltraChat training split to the full AlpacaEval dataset. 
% As shown in Fig.~\ref{fig:exp_generalization_ultrachat}, while prediction accuracy decreases compared to in-dataset testing, the predictions maintain significant correlation with true values as measured by Spearman, Kendall, and Pearson coefficients. This suggests the probes capture both dataset-specific and generalizable patterns.






% \textbf{Insight 3: Structure attribute patterns peak in middle layers for all models.} To measure the saliency of structure attribute patterns in each hidden layer, we evaluated layer-wise probing performance on UltraChat, optimizing probe hidden sizes through grid search. Fig.~\ref{fig:exp_layerHeatmap_ultrachat} shows correlation coefficients (Spearman, Kendall, Pearson) across layers, revealing a distinctive pattern: \textbf{weak performance in early layers, peaks in middle layers, and decline in final layers}. This suggests response length information builds up through early layers, reaches maximum representation in middle layers, then partially diminishes. These results also highlight that \textbf{structure attributes emerge through complex transformations across layers, beyond simple projections from vocabulary statistics}.

% \textbf{Layer-level analysis.} To identify which model layers best encode response length, we evaluate layer-wise probing performance on UltraChat. For each layer, we grid search probe hidden sizes to find the optimal configuration across seeds.
% The heatmap in Fig.~\ref{fig:exp_layerHeatmap_ultrachat} shows average correlation coefficients (Spearman, Kendall, Pearson) across layers. Probing performance follows a distinctive pattern: weak in early layers, peaks in middle layers, and declines in final layers. This pattern suggests that response length information is progressively built up through early layers, maximally represented in middle layers, and partially discarded in final layers. These results also demonstrate the value of probing LLM representations over raw embeddings, highlighting the transformers' role in pattern encoding.

% \textbf{Insight 4: Structure attribute patterns are salient and can be extracted adequately by simple and shallow MLPs.} We analyze how probe hidden size affects performance by plotting average correlation coefficients (Spearman, Kendall, Pearson) across layers for each hidden size configuration. As shown in Fig.~\ref{fig:exp_statistical_hiddensize}, performance plateaus at moderate hidden sizes, suggesting these patterns are readily accessible without complex probing architectures.

% \textbf{Probe complexity analysis.} We analyze how probe hidden size affects performance by plotting average correlation coefficients (Spearman, Kendall, Pearson) across all layers for each hidden size configuration. As shown in Fig.~\ref{fig:exp_statistical_hiddensize}, performance initially increases with probe complexity, reaching a plateau at moderate hidden sizes. Beyond this point, performance stabilizes or slightly decreases, suggesting that simpler architectures are sufficient to capture the underlying patterns while more complex probes risk overfitting.



% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/exp_generalizationResults_ultrachat_To_alpaca_eval_spearman.pdf}
%     \caption{Generalization test from ultrachat to apacal\_eval on token length prediction task.}
%     \label{fig:exp_generalization_ultrachat}
% \end{figure}




\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_ultrachat_spearman.pdf}
        \caption{Ultrachat}
        \label{fig:exp_basicResults_ultrachat}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_gsm8k_spearman.pdf}
        \caption{gsm8k}
        \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{Hidden size analysis on ultrachat and gsm8k, spearman correlation as metric}
    \label{fig:exp_statistical_hiddensize}
\end{figure*}








\subsection{Content Attributes: Character Choices and Multiple-Choice Answers}

\textbf{Insight 5: Content attribute patterns demonstrate robust classification performance, cross-dataset generalization, and accessibility.} Probing experiments on content attributes parallel our structure attribute findings: \textbf{(1)} Both base and fine-tuned models encode content information significantly above random baselines in in-dataset evaluation, \textbf{(2)} probes maintain above-baseline performance in cross-dataset settings, and \textbf{(3)} content patterns, like structure attributes, can be effectively extracted using simple MLPs with hidden size 32.

\textbf{Insight 6: Content attribute patterns peak in late layers.} Fig.~\ref{fig:exp_layerHeatmap_TinyStories} shows layer-wise pattern saliency using F1 scores, revealing that content attribute performance either remains low until late layers or gradually increases to peak in final layers, contrasting with the mid-layer peaks observed for structure attributes.


% \textbf{Task settings.} 
% Story character choice (5 classes) and multiple-choice answer (4 classes) are classification tasks evaluated using F1 score and accuracy. For story character choice, we use 10K TinyStories (in-dataset) and 10K ROCStories (cross-dataset). For multiple-choice answer, we evaluate on 10K CommonsenseQA questions. We conduct in-dataset evaluation for both tasks, with further analysis focusing on story character choice. All results are averaged across three random seeds.
% Here, we describe our data collection and labeling methods for two classification tasks that predict model performance using external ground truth labels. For answer confidence, we use 8k multiple-choice questions from MedMCQA, a challenging dataset providing more balanced success-fail ratios for tested models. We label responses as 1 if they match the ground-truth answer and 0 otherwise, then balance the classes. For factual consistency, we use 10k challenging true/false statements from CREAK dataset that are difficult to verify as true or false, asking models to indicate support or disagreement. We label responses as 1 if models correctly support true statements or reject false ones, and 0 otherwise, followed by class balancing.

% \textbf{Insight 5: Content attribute patterns demonstrate robust classification performance, cross-dataset generalization, and accessibility.} Probing experiments on content attributes (using TinyStories, CommonsenseQA, and ROCStories datasets) reveal patterns that parallel our structure attribute findings: \textbf{(1)} Both base and fine-tuned models encode content information significantly above random baselines, though base models show higher variance \textbf{(2)} Probes maintain above-baseline performance in cross-dataset evaluation (TinyStories → ROCStories), indicating generalization of learned patterns \textbf{(3)} Like structure attributes, content patterns can be effectively extracted using simple MLPs with moderate hidden sizes, suggesting these representations are readily accessible.


% \textbf{Insight 5: Probes achieve robust classification performance on content attributes in base and fine-tuned models.} We evaluate in-dataset performance on TinyStories and CommonsenseQA using different train-test splits. Fig.~\ref{fig:exp_statistical_ContentResults} shows both fine-tuned and base models achieve F1 scores and accuracies significantly above random baselines, while base models show slightly higher variance across seeds. \textbf{This indicates that emergent planning for content attribute occurs in both base and fine-tuned models}.
% \textbf{In-dataset results.} 
% We evaluate performance using different train-test splits on TinyStories and CommonsenseQA datasets. 
% As shown in Fig.~\ref{fig:exp_statistical_ContentResults}, both fine-tuned and base models achieve F1 scores and accuracies well above random baselines. Base models exhibit higher variance across seeds, but all models demonstrate encoded content attributes in their representations.


% \textbf{Insight 6: The learned content attributes generalize across datasets.} To evaluate cross-dataset generalization, we apply probes trained on TinyStories to ROCStories. Fig.~\ref{fig:exp_generalization_TinyStories} shows that while accuracy decreases compared to in-dataset testing, performance remains significantly above baselines, suggesting probes capture both dataset-specific and task-general patterns.
% \textbf{Cross-dataset generalization Results.} We evaluate generalization by applying probes trained on the TinyStories training split to the full ROCStories dataset. 
% As shown in Fig.~\ref{fig:exp_generalization_TinyStories}, while accuracy decreases compared to in-dataset testing, performance remains significantly above baselines, suggesting probes capture both dataset-specific and generalizable features.

% \textbf{Insight 6: Content attribute patterns form in late layers.} We evaluate layer-wise probing performance on TinyStories to measure the saliency of structure attribute patterns across layers, optimizing probe hidden sizes through grid search. Fig.~\ref{fig:exp_layerHeatmap_TinyStories} shows F1 scores across layers, revealing a gradual increase in pattern strength from early to final layers, where it peaks. This suggests structure attributes accumulate throughout the model's depth, reaching maximum representation in final layers.

% \textbf{Insight 8: Content attribute patterns can be extracted adequately by simple and shallow MLPs.} We analyze how probe hidden size affects performance by plotting F1 scores across layers for each hidden size configuration. As shown in Fig.~\ref{fig:exp_content_hiddensize}, performance plateaus at moderate hidden sizes, suggesting these patterns are readily extractable with moderately-sized probing architectures.
 
\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_TinyStories_f1_score.pdf}
        \caption{TinyStories}
        \label{fig:exp_basicResults_TinyStories}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_commonsense_qa_f1_score.pdf}
        \caption{commonsense\_qa}
        \label{fig:exp_basicResults_commensense_qa}
    \end{subfigure}
    \caption{Results on TinyStories and commonsense\_qa, l1 score as metric}
    \label{fig:exp_statistical_ContentResults}
\end{figure*}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/exp_generalizationResults_TinyStories_To_ROCStories_f1_score.pdf}
    \caption{Generalization test from TinyStories to ROCStories on character choices task.}
    \label{fig:exp_generalization_TinyStories}
\end{figure}

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/exp_layerHeatmap_TinyStories_f1_score.pdf}
    \caption{Layer-wise F1 score distribution across different language models on the TinyStories dataset. The heatmap shows F1 scores for each layer (x-axis) of various model architectures. Higher scores (darker red) indicate better performance. The results demonstrate that performance generally improves in higher layers, with most models showing peak F1 scores in their later layers.}
    \label{fig:exp_layerHeatmap_TinyStories}
\end{figure*}


\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_TinyStories_f1_score.pdf}
        \caption{TinyStories}
        % \label{fig:exp_basicResults_ultrachat}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_commonsense_qa_f1_score.pdf}
        \caption{commonsense\_qa}
        % \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{Hidden size analysis on TinyStories and commonsense\_qa, f1 score as metric}
    \label{fig:exp_content_hiddensize}
\end{figure*}





\subsection{Behavior Attributes: Answer Confidence and Factual Consistency}

\textbf{Insight 7: Behavior attribute patterns exhibit strong classification accuracy, cross-dataset transferability, and accessibility.} Probing experiments on behavior attributes parallel our previous findings: \textbf{(1)} Both base and fine-tuned models encode behavior information (Fig.~\ref{fig:ex}), \textbf{(2)} probes maintain above-baseline performance when transferring from MedMCQA to ARC-Challenge, and \textbf{(3)} behavior patterns, like structure and content attributes, can be effectively extracted using simple MLPs.

% \textbf{Insight 7: Behavior attribute patterns exhibit strong classification accuracy, cross-dataset transferability, and accessibility in their representations.} Probing experiments on behavior attributes (using MedMCQA and ARC-Challenge datasets) reveal patterns that parallel our previous findings: \textbf{(1)} Both base and fine-tuned models encode behavior information with above-baseline F1 scores and accuracies \textbf{(2)} Probes maintain significant above-baseline performance in cross-dataset evaluation (MedMCQA → ARC-Challenge), demonstrating generalization of learned patterns \textbf{(3)} Like structure and content attributes, behavior patterns can be effectively extracted using simple MLPs with moderate hidden sizes, indicating accessible representations.


\textbf{Insight 8: Behavior attribute patterns accumulate and peak in different layers between models.} Evaluating layer-wise probe performance on MedMCQA reveals F1 scores gradually increase through model depth, peaking near final layers, though some models show slight performance decline in the very last layer. This suggests behavior attributes, like structure attributes, accumulate progressively through the network's layers.

% \textbf{Task settings.} 
% Answer confidence and factual consistency are binary classification tasks evaluated with F1 score and accuracy. We test answer confidence on 10K MedMCQA questions (in-dataset) and 2.6K ARC-Challenge questions (cross-dataset), while factual consistency is evaluated on 10K CREAK statements. We perform in-dataset testing for both tasks and include additional analysis on story character choice. All results are averaged across three random seeds.


% \textbf{Insight 9: Probes achieve robust classification performance on behavior attributes in base and fine-tuned models.} We evaluate in-dataset performance on MedMCQA and ARC-Challenge using different train-test splits. Fig.~\ref{fig:exp_statistical_BehaviorResults} shows both fine-tuned and base models achieve F1 scores and accuracies significantly above random baselines. This indicates that emergent planning for behavior attributes occurs in both base and fine-tuned models.
% \textbf{In-dataset results.} 
% We evaluate performance using train-test splits on MedMCQA and ARC-Challenge datasets. As shown in Fig.~\ref{fig:exp_statistical_BehaviorResults}, both fine-tuned and base models achieve F1 scores and accuracies significantly above random baselines, suggesting their representations effectively encode behavior attributes.

% \textbf{Insight 10: The learned behavior attributes generalize across datasets.} To evaluate cross-dataset generalization, we applied probes trained on MedMCQA to ARC-Challenge. Fig.~\ref{fig:exp_generalization_medmcqa} shows that while accuracy decreases compared to in-dataset testing, performance remains significantly above random baselines, suggesting probes capture both dataset-specific and task-general features.

% \textbf{Cross-dataset generalization results.} 
% We evaluate generalization by applying probes trained on the MedMCQA training split to the full ARC-Challenge dataset. As shown in Fig.~\ref{fig:exp_generalization_medmcqa}, while accuracy decreases compared to in-dataset testing, performance remains above random baselines.

% \textbf{Insight 11: Behavior attribute patterns peak in final layers.} To measure the saliency of behavior attribute patterns across layers, we evaluated layer-wise probing performance on MedMCQA, optimizing probe hidden sizes through grid search. Fig.~\ref{fig:exp_layerHeatmap_medmcqa} shows F1 scores across layers, revealing a gradual increase in pattern strength toward final layers, with some models showing slight degradation at the very end. This suggests behavior attributes accumulate throughout the model's depth, reaching maximum representation near final layers.
% \textbf{Layer-level analysis.} 
% We evaluate layer-wise probing performance on MedMCQA.
% Are shown in Fig.~\ref{fig:exp_layerHeatmap_medmcqa}, the heatmap of averaged k1 scores reveals that encoding strength gradually increases through the network, typically peaking near or at the final layers, though some models show slight degradation at the very end. This suggests behavior attributes accumulate progressively through the model's depth.

% \textbf{Insight 12: Behavior attribute patterns  can be extracted adequately by simple and shallow MLPs.} We analyze how probe hidden size affects performance by plotting F1 scores across layers for each hidden size configuration. As shown in Fig.~\ref{fig:exp_main_behavior_hiddensize}, performance plateaus at moderate hidden sizes, suggesting these patterns are readily extractable with moderately-sized probing architectures.

% \textbf{Probe complexity analysis.} 
% We analyze the relationship between probe hidden size and performance by measuring average F1 scores across layers. As shown in Fig.~\ref{fig:exp_main_behavior_hiddensize}, while simple architectures yield limited performance, effectiveness improves with increased hidden size until plateauing, suggesting our probe architectures adequately capture the underlying patterns.

\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_medmcqa_f1_score.pdf}
        \caption{medmcqa}
        \label{fig:exp_basicResults_medmcqa}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_basicResults_CREAK_f1_score.pdf}
        \caption{CREAK}
        \label{fig:exp_basicResults_CREAK}
    \end{subfigure}
    \caption{Results on medmcqa and CREAK, l1 score as metric}
    \label{fig:exp_statistical_BehaviorResults}
\end{figure*}

 \begin{figure}[tb!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/exp_generalizationResults_medmcqa_To_ai2_arc-Challenge_f1_score.pdf}
    \caption{Generalization test from medmcqa to Challenge set of ai2\_arc on answer confidence task.}
    \label{fig:exp_generalization_medmcqa}
\end{figure}

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/exp_layerHeatmap_medmcqa_f1_score.pdf}
    \caption{Layer-wise F1 score distribution across different language models on the medmcqa dataset. The heatmap shows F1 scores for each layer (x-axis) of various model architectures. Higher scores (darker red) indicate better performance. The results demonstrate that performance generally improves in higher layers, with most models showing peak F1 scores in their later layers.}
    \label{fig:exp_layerHeatmap_medmcqa}
\end{figure*}

\begin{figure*}[tb!] 
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_medmcqa_f1_score.pdf}
        \caption{medmcqa}
        % \label{fig:exp_basicResults_ultrachat}
    \end{subfigure}
    \hfill  % Creates horizontal spacing between subfigures
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/exp_hiddenSizeAnalysis_CREAK_f1_score.pdf}
        \caption{CREAK}
        % \label{fig:exp_basicResults_gsm8k}
    \end{subfigure}
    \caption{Hidden size analysis on medmcqa and CREAK, f1 score as metric}
    \label{fig:exp_main_behavior_hiddensize}
\end{figure*}



% \subsection{Insights Across Tasks and Attribute Types}
% \textbf{Insight 9: Emergent planning exhibits.} xxx


% \textbf{Insight 10: Different attributes types are mainly decoded in different model layers.} Structure attributes are mainly decoded in the middle layers; content and behavior attributes peaks at finally layers.


